The Effect of Ground Truth Accuracy on the Evaluation of Localization Systems

The ability to accurately evaluate the performance of location determination systems is crucial for many applications. Typically, the performance of such systems is obtained by comparing ground truth locations with estimated locations. However, these ground truth locations are usually obtained by clicking on a map or using other worldwide available technologies like GPS. This introduces ground truth errors that are due to the marking process, map distortions, or inherent GPS inaccuracy. In this paper, we present a theoretical framework for analyzing the effect of ground truth errors on the evaluation of localization systems. Based on that, we design two algorithms for computing the real algorithmic error from the validation error and marking/map ground truth errors, respectively. We further establish bounds on different performance metrics. Validation of our theoretical assumptions and analysis using real data collected in a typical environment shows the ability of our theoretical framework to correct the estimated error of a localization algorithm in the presence of ground truth errors. Specifically, our marking error algorithm matches the real error CDF within 4%, and our map error algorithm provides a more accurate estimate of the median/tail error by 150%/72% when the map is shifted by 6m.

==> main_arXiv (1)/model.tex <==
\section{Fundamental Mathematical Model}
\label{sec:model}
\newtheorem{example}{Example}

In this section, we introduce the mathematical model used for evaluating the performance of a general location determination system and state the problems we study in this paper.

\subsection{Types of Ground Truth Errors}
First, we define two types of ground truth error: marking error and map error. In Figure \ref{fig:errors}(a), the user is at the green circle but marks his/her location at the blue triangle on an accurate map. In this case, we call the ground truth error as \textbf{\em marking error}. For example, this can be due to the lack of landmarks for the user to determine his/her exact location accurately on an open space on the map of the small screen of a mobile device, or simply due to a mistake from the user.

In Figure \ref{fig:errors}(b), the user would mark his/her location at the blue triangle if an accurate map is used. However, he/she actually marks location at the orange diamond due to using an incorrect map (as in Figure \ref{fig:japan}). In this case, we call this second ground truth error as \textbf{\em map error}.

\subsection{System Model and Problem Statement}

Next, consider a localization algorithm which returns a user's 2D location $X^{algo}$. Let $X^{gt}$ be the user's actual (real) ground truth location and $\widehat{X}^{gt}$ be the human-marked ground truth location.
Ideally we would like to calculate the algorithm's \textbf{\em real error}
$Err^{real} = X^{gt} - X^{algo}$.
However, due to the ground truth error
$Err^{gt} = \widehat{X}^{gt} - X^{gt}$,
the \textbf{\em validation error} actually used to evaluate the algorithm's performance in literature and many practical systems is
\begin{equation*}
Err^{val} = \widehat{X}^{gt} - X^{algo} = Err^{real} + Err^{gt}
\end{equation*}

Clearly, we are more interested in the location accuracy $|Err^{real}|$, rather than $|Err^{val}|$ which is impacted by the ground truth error. Once there is enough evaluation data ($\{X^{algo}, \widehat{X}^{gt}\}$), we can know the cumulative distribution function of $|Err^{val}|$. Furthermore, instead of using the full distribution, the accuracy is commonly expressed using high-level summary statistics, e.g. ``some inexpensive GPS receivers can locate positions to within 10 meters for approximately 95 percent of measurements \cite{Hightower2001}.'' In this paper, we consider three major summary statistics that are commonly used in literature and practical systems to quantify a localization algorithm performance:
\begin{itemize}
    \item The mean error $|Err^{val}|_{mean}$
    \item The 50\%-median error $|Err^{val}|_{median}$
    \item The 95\%-tail error $|Err^{val}|_{tail}$ \footnote{We select 95\% as it is most commonly used for confidence intervals \cite{Zar2007}. But in theory any level can be selected for the tail error such as 90\% or 99\%.}
\end{itemize}
The mean and median reflects the average user experience, while the tail reflects the worst user experience.

We again emphasize that, since we are more interested to know $|Err^{real}|_{mean}$ instead of $|Err^{val}|_{mean}$, we define the {\em \textbf{impact} of ground truth error}
\begin{equation}
\label{eq:delta_notion}
\Delta_{mean} = |Err^{val}|_{mean} - |Err^{real}|_{mean}
\end{equation}
as the difference between the validation error and the real error, i.e. how much of the validation error is caused by the ground truth error. The notions of $\Delta_{median}$ / $\Delta_{tail}$ are similar to (\ref{eq:delta_notion}).


\begin{figure}[t]
\vspace{-1mm}
\centerline
{\includegraphics[width=0.5\textwidth]{figures/errors.png}}
\caption{Ground truth errors. (a) A marking error between actual ground truth location (green circle) and human-marked ground truth location on an accurate map (blue triangle). (b) An additional map error between human-marked ground truth location on an accurate map (blue triangle) and that on an incorrect map (orange diamond).}
\label{fig:errors}
\end{figure}

To summarize, in this paper we propose and answer the following questions:
\begin{enumerate}
    \item Given the summary statistics on the validation error $|Err^{val}|_{mean}$ and the ground truth (marking/map) error $|Err^{gt}|_{mean}$, how can one computes the real algorithmic error $|Err^{real}|_{mean}$?
    \item What is the relation between the impact $\Delta_{mean}$ and the ground truth (marking/map) error $|Err^{gt}|_{mean}$?
    \item Can we answer the above two questions for other metrics such as the median or 95\%-tail error, or more generally for any $q$-th quantile?
    \item Which ground truth error has a larger impact on the evaluation of a localization system? Marking error or map error?
\end{enumerate}





\subsection{Application Example}
\label{sec:application}
Given a localization algorithm with validation error $|Err^{val}|_{mean} = 6m$ (which is the main metric commonly used in literature). The human-marked ground truth is collected on an incorrect map with an offset $|Err^{map}| = 2m$, and we estimate there is an average marking error $|Err^{mark}|_{mean} = 3m$.

First, we use Algorithm~\ref{algo:map} (Section \ref{sec:map_error}) to remove the map error, which gives a new validation error $|Err^{val}|_{mean} = 5.79m$ on an accurate map.
Next, we use Algorithm~\ref{algo:marking} (Section \ref{sec:marking_error}) to remove the marking error and end up with a real error $|Err^{real}|_{mean} = 4.95m$. This final error is a more realistic/accurate reflection of the algorithm performance in real time after removing the inaccuracy in ground truth collection.


==> main_arXiv (1)/theory.tex <==
\section{Theoretical Results}
\label{sec:theory}
\newtheorem{theorem}{Theorem}

Mathematically, instead of giving the summary statistics $|Err^{val}|_{mean}$ and $|Err^{gt}|_{mean}$, even if we know the full distribution of $Err^{val}$ and $Err^{gt}$, it is still hard to solve the distribution of $Err^{real}$ such that
$Err^{val} = Err^{real} + Err^{gt}$.
This is because the real algorithmic error and the ground truth error are independent, but the validation error and the ground truth error are not; and we do not know the correlation between them.

To make the problem mathematically tractable, we assume that the algorithmic and marking errors follow the most widely used normal distributions. We also further consider the map error of a constant translation. %

We start by analyzing the marking error in Section~\ref{sec:marking_error} and map error in Section~\ref{sec:map_error}. We then compare these two errors in Section~\ref{sec:compare_error}, and discuss the \textit{map scale error} in Section~\ref{sec:scale_error}. All assumptions are validated in Section~\ref{sec:evaluation}.

\subsection{Marking Error}
\label{sec:marking_error}

\begin{algorithm}[t]
\caption{Compute the real error from validation error and marking error. This algorithm uses mean but can be extended to any $q$-th quantile ($0 < q < 1$).}
\label{algo:marking}
\begin{algorithmic}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\REQUIRE validation error mean $u = |Err^{val}|_{mean}$, marking error mean $v = |Err^{mark}|_{mean}$, $u > v$
\ENSURE real error mean $|Err^{real}|_{mean}$
\RETURN $|Err^{real}|_{mean} = \sqrt{u ^ 2 - v ^ 2}$
\end{algorithmic}
\end{algorithm}

Assume that both the real algorithmic error and the marking error follow 2D Gaussian distributions\footnote{We write $diag[{\sigma} ^ 2]$ for short to represent a matrix that has ${\sigma} ^ 2$ on all diagonal entries and zero otherwise.}
$Err^{real} \sim \mathcal{N}(0, diag[(\sigma^{real}) ^ 2])$,
$Err^{mark} \sim \mathcal{N}(0, diag[(\sigma^{mark}) ^ 2])$.
We also assume that both error distributions are symmetric in 2D (do not have any orientation bias), so that they have zero mean and the errors in X and Y directions are independent and identically distributed. In this setting, the validation error is also a 2D Gaussian
\begin{equation*}
Err^{val} = Err^{real} + Err^{mark} \sim \mathcal{N}(0, diag[(\sigma^{val})^2])
\end{equation*}
where
$(\sigma^{val}) ^ 2 = (\sigma ^ {real}) ^ 2 + (\sigma^{mark}) ^ 2$.

For the 1D error norm, it is known that for a Gaussian variable $X \sim \mathcal{N}(0, diag[{\sigma}^2])$, its norm $|X|$ follows a distribution $|X| \sim Rayleigh(\sigma)$ \cite{Rayleigh1880} with a probability density function
$p(x | \sigma) = \frac{x}{\sigma^{2}} e^{-\frac{x^2}{2 \sigma^2}}$, $x \geq 0$
and its mean $|X|_{mean}$ is equal to
$Rayleigh(\sigma)_{mean} = \sigma \sqrt{\pi / 2}$.

Thus $|Err^{mark}|$, $|Err^{real}|$ and $|Err^{val}|$ are all Rayleigh distributions. Since the mean is linear in $\sigma$,
\begin{align}
|Err^{real}|_{mean} & = \sigma^{real} \sqrt{\pi / 2} = \sqrt{\left( (\sigma^{val}) ^ 2 - (\sigma^{mark}) ^ 2 \right) \pi / 2} \nonumber \\
& = \sqrt{|Err^{val}|_{mean} ^ 2 - |Err^{mark}|_{mean} ^ 2} \label{eq:real_mean}
\end{align}

Algorithm~\ref{algo:marking} shows how to obtain the real error mean given the validation and marking error means. It also applies to the median and 95\%-tail, because for any $q$-th quantile ($0 < q < 1$),
$Rayleigh(\sigma)_{q \text{-th}} = \sigma \sqrt{-2 \ln{(1 - q)}}$
is always linear in $\sigma$.

\begin{figure}[t]
\vspace{-2mm}
\centerline
{\includegraphics[width=0.25\textwidth]{figures/impact_marking.png}}
\caption{Impact of marking error $\Delta_{mean}$ as a function of $|Err^{val}|_{mean}$ and $|Err^{mark}|_{mean}$. The figures for $\Delta_{median}$ / $\Delta_{tail}$ are similar.}
\label{fig:impact_marking}
\vspace{-2mm}
\end{figure}

\begin{theorem}
\label{thm:impact_marking}
The impact of marking error ($\Delta_{mean}$):
\begin{equation*}
\frac{|Err^{mark}|_{mean}^2}{2 |Err^{val}|_{mean}} < \Delta_{mean}
< \frac{|Err^{mark}|_{mean}^2}{2 |Err^{val}|_{mean} - |Err^{mark}|_{mean}}
\end{equation*}
This also holds if we replace the mean by any $q$-th quantile (e.g. $\Delta_{median}$ and $\Delta_{tail}$).
\end{theorem}

\begin{proof}
From (\ref{eq:real_mean}),
$|Err^{val}|_{mean} - |Err^{mark}|_{mean} < |Err^{real}|_{mean} < |Err^{val}|_{mean}$.
\begin{align*}
\Delta_{mean} & = |Err^{val}|_{mean} - |Err^{real}|_{mean} \\
& = \frac{|Err^{val}|_{mean}^2 - |Err^{real}|_{mean}^2}{|Err^{val}|_{mean} + |Err^{real}|_{mean}} \\
& = \frac{|Err^{mark}|_{mean}^2}{|Err^{val}|_{mean} + |Err^{real}|_{mean}}
\end{align*}
\begin{equation*}
\frac{|Err^{mark}|_{mean}^2}{2 |Err^{val}|_{mean}} < \Delta_{mean}
< \frac{|Err^{mark}|_{mean}^2}{2 |Err^{val}|_{mean} - |Err^{mark}|_{mean}}
\end{equation*}
\end{proof}

Theorem \ref{thm:impact_marking} gives us a direct quantitative measure on the impact of marking error on location accuracy (see Figure~\ref{fig:impact_marking}):
\begin{enumerate}
    \item $\Delta$ is quadratic in $|Err^{mark}|$. This means that a small error in the collected ground truth has a magnified (quadratic) impact on the error in the reported algorithm accuracy. %
    \item $\Delta$ is inversely proportional to $|Err^{val}|$, i.e. when a localization algorithm does not perform well on validation, the impact of marking error is not significant. As the algorithm improves to have better accuracy, the quality of ground truth data becomes more and more important.
\end{enumerate}

\begin{theorem}
\label{thm:tail_median}
Relations between the real error mean, median, and 95\%-tail.
\begin{equation*}
\frac{|Err^{real}|_{tail}}{|Err^{real}|_{median}} = 2.07 ~ \textrm{and} ~
\frac{|Err^{real}|_{tail}}{|Err^{real}|_{mean}} = 1.95
\end{equation*}
These also hold if we replace $|Err^{real}|$ by $|Err^{val}|$.
\end{theorem}

\begin{proof}
\begin{align*}
\frac{|Err^{real}|_{tail}}{|Err^{real}|_{median}} & = \frac{\sigma^{real} \sqrt{-2 \ln{(1 - 0.95)}}}{\sigma^{real} \sqrt{-2 \ln{(1 - 0.5)}}} = 2.07 \\
\frac{|Err^{real}|_{tail}}{|Err^{real}|_{mean}} & = \frac{\sigma^{real} \sqrt{-2 \ln{(1 - 0.95)}}}{\sigma^{real} \sqrt{\pi / 2}} = 1.95
\end{align*}
\end{proof}

Theorem \ref{thm:tail_median} gives us an approximation on the average/worst user experience on location accuracy, e.g. if a GPS receiver has an accuracy of 10 meters for 95\% of the time, we would expect that it can localize within 5 meters for 50\% of the time.

\subsection{Map Error (Translation)}
\label{sec:map_error}

\begin{figure}[t]
\vspace{-1mm}
\centerline
{\includegraphics[width=0.25\textwidth]{figures/delta.png}}
\caption{$\Delta_{mean}(v, 1)$ approximation function. $\Delta(v, 1)$ values are calculated by using the numerical Bessel function \cite{Schwartz2012}. $\delta(v, 1)$ values are calculated by using the algebraic approximation function. The figures for $\Delta_{median}$ / $\Delta_{tail}$ are similar.}
\label{fig:delta}
\end{figure}

Again, we assume that %
$Err^{real} \sim \mathcal{N}(0, diag[(\sigma^{real})^2])$
but
$Err^{map} = V$
is a constant 2D vector.
For now we assume that there is no marking error (see Section \ref{sec:application} when both marking and map errors exist). In this setting, the validation error is also a 2D Gaussian but with a non-zero mean
\begin{equation*}
Err^{val} = Err^{real} + Err^{map} \sim \mathcal{N}(V, diag[(\sigma^{real})^2])
\end{equation*}

For simplicity, let $\sigma = \sigma^{real}$ since there is only one variance parameter in this section (as the map error is a constant), and $v = |V|$ be the norm of the map error vector. The 1D error norm
$|Err^{real}| \sim Rayleigh(\sigma)$, $|Err^{map}| = v$.

For a non-zero mean Gaussian variable $X \sim \mathcal{N}(V, diag[{\sigma}^2])$, its norm $|X|$ follows a distribution $|X| \sim Rice(v, \sigma)$ \cite{Rice1944} with a probability density function
$p(x | v, \sigma) = \frac{x}{\sigma ^ 2} e ^ {- \frac{x ^ 2 + v ^ 2}{2 \sigma ^ 2}} I_0 \left( \frac{xv}{\sigma ^ 2} \right)$, $x \geq 0$
where
$I_0(z) = \sum_{k = 0}^{\infty} \frac{(z / 2) ^ {2k}}{(k!) ^ 2}$
is the modified Bessel function of the first kind with order zero.
Note that when $v = 0$, $Rice(v, \sigma)$ is the same as $Rayleigh(\sigma)$.

Finally, the impact of map error is
\begin{align*}
\Delta_{mean}(v, \sigma) & = |Err^{val}|_{mean} - |Err^{real}|_{mean} \\
& = Rice(v, \sigma)_{mean} - Rice(0, \sigma)_{mean}
\end{align*}
and similarly for $\Delta_{median}$ / $\Delta_{tail}$.

\subsubsection{$\Delta(v, \sigma)$ Approximation Function}

\begin{table}[t]
\caption{Constants $\alpha$, $\beta$ for $\delta(v, 1)$ approximation function and root-mean-square error on $|\Delta(v, 1) - \delta(v, 1)|$.}
\begin{center}
\vspace{-1mm}
\begin{tabular}{|c|c|c|c|}
\hline
 & $\alpha$ & $\beta$ & $RMSE~|\Delta - \delta|$ \\
\hline
$\text{Mean}$ & 1.2392 & 2.3064 & 0.0052 \\
$\text{Median}$ & 1.1471 & 2.3384 & 0.0032 \\
$\text{Tail}$ & 0.7870 & 1.9452 & 0.0038 \\
\hline
\end{tabular}
\label{table:alpha_beta}
\end{center}
\end{table}

\begin{table}[t]
\caption{Constant $\gamma$ for $Rice(0, 1)/Rayleigh(1)$.}
\vspace{-1mm}
\begin{center}
\begin{tabular}{|c|c|}
\hline
 & $\gamma$ \\
\hline
$\text{Mean}$ & $\sqrt{\pi / 2} = 1.2533$ \\
$\text{Median}$ & $\sqrt{-2 \ln{(1 - 0.5)}} = 1.1774$ \\
$\text{Tail}$ & $\sqrt{-2 \ln{(1 - 0.95)}} = 2.4477$ \\
\hline
\end{tabular}
\label{table:gamma}
\end{center}
\vspace{-1mm}
\end{table}

Unlike Rayleigh distribution, the mean/quantile statistics of Rice distribution have no closed-form expressions. This is because in general, Bessel functions cannot be expressed as a finite algebraic combination of elementary functions \cite{Ritger1968}. To make the analysis easier, we give an algebraic approximation function for computing the impact $\Delta(v, \sigma)$.

We start with analysis on the mean error. By scaling a factor of $1/\sigma$, we have
\begin{align}
\Delta(v, \sigma) & = Rice(v, \sigma)_{mean} - Rice(0, \sigma)_{mean} \nonumber \\
& = \sigma \left( Rice(v / \sigma, 1)_{mean} - Rice(0, 1)_{mean} \right) \nonumber \\
& = \sigma \Delta (v / \sigma, 1) \label{eq:delta_scale}
\end{align}

Consider the function
\begin{equation*}
\Delta(v, 1) = Rice(v, 1)_{mean} - Rice(0, 1)_{mean}
\end{equation*}
where
$Rice(0, 1)_{mean} = Rayleigh(1)_{mean} = \sqrt{\pi / 2}$.

It has the following two properties:
\begin{itemize}
    \item $\Delta(0, 1) = 0$
    \item $\lim_{v \to \infty} \frac{\Delta(v, 1)}{v} = 1$ \footnote{As $v \to \infty$, if v increases by 1, the norm $|X|$ of every sample $X \sim Rice(v, 1)$ increases by an amount that also converges to 1. Thus $\Delta(v, 1)$ is linear in $v$ with slope 1.}
\end{itemize}

We next construct an algebraic approximation function
\begin{equation}
\label{eq:approx_func}
\delta(v, 1) = (v ^ \beta + \alpha ^ \beta) ^ \frac{1}{\beta} - \alpha
\end{equation}
with two rational number constants $\alpha > 0$, $\beta > 1$. Here $\alpha$ sets the difference between $v$ and $\delta(v, 1)$ as $v \to \infty$, and $\beta$ controls how $\delta(v, 1)$ varies for small $v$.
One can verify that $\delta(v, 1)$ has two similar properties:
\begin{itemize}
    \item $\delta(0, 1) = 0$
    \item $\lim_{v \to \infty} \frac{\delta(v, 1)}{v} = 1$
\end{itemize}

Figure \ref{fig:delta} shows a comparison of $\Delta(v, 1)$ and its approximation $\delta(v, 1)$. The $\Delta(v, 1)$ values are computed by generating the probability density function using numerical calculations of the Bessel function \cite{Schwartz2012}, and the approximation $\delta(v, 1)$ values are computed from the closed-form expression (\ref{eq:approx_func}). The constants $\alpha$ and $\beta$ are optimized to minimize the root-mean-square error on $|\Delta(v, 1) - \delta(v, 1)|$ (see Table \ref{table:alpha_beta}).

Once we have $\delta(v, 1)$, similar to (\ref{eq:delta_scale})
\begin{equation*}
\delta(v, \sigma) = \sigma \delta (v / \sigma, 1) = \sigma \left( \left( (v / \sigma) ^ \beta + \alpha ^ \beta \right) ^ {\frac{1}{\beta}} - \alpha \right)
\end{equation*}

\subsubsection{Numerical Algorithm for Computing the Real Error (Algorithm \ref{algo:map})}

\begin{algorithm}[t]
\caption{Compute the real error from validation error and map error. This algorithm uses mean but can be extended to any $q$-th quantile ($0 < q < 1$).}
\label{algo:map}
\begin{algorithmic}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\REQUIRE validation error mean $u = |Err^{val}|_{mean}$, map error $v = |Err^{map}|$, $u > v$
\ENSURE real error mean $|Err^{real}|_{mean}$
  \STATE Find $\alpha, \beta$ for mean error in Table \ref{table:alpha_beta}, and $\gamma$ in Table \ref{table:gamma}
  \STATE Set $\sigma_{min} = (u - v) / \gamma$, $\sigma_{max} = (u - v) / (\gamma - \alpha)$
  \STATE Set $\epsilon$ for convergence
  \WHILE {$\sigma_{max} - \sigma_{min} > \epsilon$}
    \STATE $\sigma = (\sigma_{min} + \sigma_{max}) / 2$
    \IF {$(u / \sigma + \alpha - \gamma) ^ \beta - (v / \sigma) ^ \beta - \alpha ^ \beta < 0$}
      \STATE $\sigma_{max} = \sigma$
    \ELSE
      \STATE $\sigma_{min} = \sigma$
    \ENDIF
  \ENDWHILE
\RETURN $|Err^{real}|_{mean} = \sigma \gamma$
\end{algorithmic}
\end{algorithm}

Using the $\Delta(v, \sigma)$ approximation function, we can obtain the real error mean as follows:

Let $u = |Err^{val}|_{mean}$, $\gamma = Rice(0, 1)_{mean} = \sqrt{\pi / 2}$.
By definition of $\Delta_{mean}$,
\begin{align*}
|Err^{val}|_{mean} & = |Err^{real}|_{mean} + \Delta(v, \sigma) \\
u & = \sigma \gamma + \sigma \left( \left( (v / \sigma) ^ \beta + \alpha ^ \beta \right) ^ \frac{1}{\beta} - \alpha \right)
\end{align*}

This is equivalent to solving the equation
\begin{equation}
\label{eq:solve_sigma}
f(\sigma) = (u / \sigma + \alpha - \gamma) ^ \beta - (v / \sigma) ^ \beta - \alpha ^ \beta = 0
\end{equation}

Let $\sigma_{min} = \frac{u - v}{\gamma}$, $\sigma_{max} = \frac{u - v}{\gamma - \alpha}$.
\begin{align*}
f(\sigma_{min}) & = (v / \sigma_{min} + \alpha) ^ \beta - (v / \sigma_{min}) ^ \beta - \alpha ^ \beta > 0 \\
f(\sigma_{max}) & = - \alpha ^ \beta < 0
\end{align*}

and $\forall{\sigma < \sigma_{max}}$,
\begin{equation*}
f'(\sigma) = - \beta \left( (u / \sigma + \alpha - \gamma) ^ {\beta - 1} - (v / \sigma) ^ {\beta - 1} \right) \Big/ {\sigma^2} < 0
\end{equation*}

Therefore, we can binary search on $\sigma \in (\sigma_{min}, \sigma_{max})$ to solve $f(\sigma) = 0$. Finally,
$|Err^{real}|_{mean} = \sigma \gamma$.

Figure \ref{fig:impact_map} shows the impact of map error $\Delta(v, \sigma)$, which seems to increase slower (comparing to marking error) until when the map error $v$ is close to the validation error $u$. Intuitively, this can be explained as follows:
Let the real error be a zero mean Gaussian centered at the origin $O$, and we add a map error $V = (v, 0)$, where $v > 0$.
For any sample $X$, its error increases $|X - V| > |X - O|$ if and only if $X$ lies on the left side of the line $x = v / 2$.
Since the Gaussian has zero mean, there are more samples on the left side of the line $x = v / 2$, so the overall mean error will increase. But it increases slowly as the changes on two sides may cancel each other, until for sufficiently large $v$ where a significant majority of samples are on the left side of the line $x = v / 2$.

Similarly, Algorithm~\ref{algo:map} can be applied to any $q$-th quantile ($0 < q < 1$). Table~\ref{table:alpha_beta} and \ref{table:gamma} also list $\alpha$, $\beta$, and $\gamma$ values for the median and 95\%-tail.

Note that unlike marking error, for map error, Theorem~\ref{thm:tail_median} only holds for the real error
$\frac{|Err^{real}|_{tail}}{|Err^{real}|_{median}} > 2$,
but not for the validation error as
$\lim_{v \to \infty} \frac{|Err^{val}|_{tail}}{|Err^{val}|_{median}} = \lim_{v \to \infty} \frac{|Err^{real}|_{tail} + \Delta_{tail}(v, \sigma)}{|Err^{real}|_{median} + \Delta_{median}(v, \sigma)} = 1$, because $\lim_{v \to \infty} \frac{\Delta(v, \sigma)}{v} = 1$.

\begin{figure}[t]
\centerline
{\includegraphics[width=0.25\textwidth]{figures/impact_map.png}}
\caption{Impact of map error $\Delta_{mean}$ as a function of $|Err^{val}|_{mean}$ and $|Err^{map}|$. These curves are similar to Fig.~\ref{fig:impact_marking} on the marking error, but values are smaller.}
\label{fig:impact_map}
\end{figure}


\subsection{Comparing the Impact of Marking and Map Errors}
\label{sec:compare_error}

In Section~\ref{sec:map_error}, we briefly explained that the impact of map error is less than marking error on $\Delta_{mean}$, when the map error is equal to the marking error mean. Now we formally prove this result.

\begin{theorem}
\label{thm:impact_compare}
Given the validation error $u = |Err^{val}|_{mean}$ and the ground truth error $v = |Err^{gt}|_{mean}$ (either marking or map error), $u > v$. Let $\Delta_{mean}^{mark}$ be the impact of marking error when $v$ is $|Err^{mark}|_{mean}$, and $\Delta_{mean}^{map}$ be the impact of map error when $v$ is $|Err^{map}|$. With similar definitions on $\Delta_{median}$ / $\Delta_{tail}$, we have
\begin{align*}
& \Delta_{mean}^{mark} > \Delta_{mean}^{map}, ~ \forall{v / u < 0.9995} \\
& \Delta_{median}^{mark} > \Delta_{median}^{map}, ~ \forall{v / u < 0.9970} \\
& \Delta_{tail}^{mark} < \Delta_{tail}^{map}
\end{align*}
\end{theorem}

\begin{proof}
We start with $\Delta_{mean}$. From Algorithm~\ref{algo:marking}, $\Delta_{mean}^{mark} = u - \sqrt{u ^ 2 - v ^ 2}$. From Algorithm \ref{algo:map}, $\Delta_{mean}^{map} = u - \sigma^{*} \gamma$ where $\sigma^{*} \in (\sigma_{min}, \sigma_{max})$ is the solution for $f(\sigma) = 0$ in (\ref{eq:solve_sigma}).

So $\Delta_{mean}^{mark} > \Delta_{mean}^{map}$ if and only if
\begin{equation}
\label{eq:proof_sigma}
\sigma^{*} > \sqrt{u ^ 2 - v ^ 2} \Big/ \gamma
\end{equation}

Let $s = \sqrt{\frac{u + v}{2}}$, $t = \sqrt{\frac{u - v}{2}}$, $\lambda = t / s < 1$.

Then $u = s^2 + t^2$, $v = s^2 - t^2$, $\frac{v}{u} = \frac{1 - \lambda^2}{1 + \lambda^2}$.

(a) When $\lambda = \frac{t}{s} \le \frac{\gamma - \alpha}{\gamma}$, i.e. $\frac{v}{u} \ge \frac{1 - \left( \frac{\gamma - \alpha}{\gamma} \right)^2}{1 + \left( \frac{\gamma - \alpha}{\gamma} \right)^2} = 0.9997$,
\begin{equation*}
\frac{\sqrt{u ^ 2 - v ^ 2}}{\gamma} = \frac{2st}{\gamma} \ge \frac{2t^2}{\gamma - \alpha} = \frac{u - v}{\gamma - \alpha} = \sigma_{max} > \sigma^{*}
\end{equation*}

In this case, $\Delta_{mean}^{mark} < \Delta_{mean}^{map}$.

(b) When $\lambda = \frac{t}{s} > \frac{\gamma - \alpha}{\gamma}$, i.e. $\frac{v}{u} < 0.9997$,
\begin{equation*}
\sqrt{u ^ 2 - v ^ 2} \Big/ \gamma < \sigma_{max}, ~ \sigma^{*} < \sigma_{max}
\end{equation*}

Since $\forall{\sigma < \sigma_{max}}$, $f'(\sigma) < 0$. (\ref{eq:proof_sigma}) is equivalent to
\begin{equation*}
f \left( \sqrt{u ^ 2 - v ^ 2} \Big/ \gamma \right) > f(\sigma^{*}) = 0 \end{equation*}
\begin{equation*}
\left( \frac{u}{\frac{\sqrt{u ^ 2 - v ^ 2}}{\gamma}} + \alpha - \gamma \right) ^ \beta - \left( \frac{v}{\frac{\sqrt{u ^ 2 - v ^ 2}}{\gamma}} \right) ^ \beta - \alpha ^ \beta > 0
\end{equation*}

Replace $(u, v)$ by $(s, t)$,
\begin{equation*}
\left( \frac{s^2 + t^2}{2st} + \frac{\alpha}{\gamma} - 1 \right) ^ \beta - \left( \frac{s^2 - t^2}{2st} \right) ^ \beta - \left( \frac{\alpha}{\gamma} \right) ^ \beta > 0
\end{equation*}

Using $\lambda = t / s$,
\begin{align}
g(\lambda) & = \left( 1 + 2 \lambda (\alpha / \gamma - 1) + \lambda^2 \right) ^ \beta - (1 - \lambda^2) ^ \beta - ( 2 \lambda \alpha / \gamma) ^ \beta \nonumber \\
& > 0 \label{eq:lambda}
\end{align}

Figure \ref{fig:lambda} plots the algebraic function $g(\lambda)$ and its derivative $g'(\lambda)$ on $0 \le \lambda \le 1$. They satisfy
\begin{align*}
& g(0) = 0, ~ g'(0) = 2 \beta ( \alpha / \gamma - 1 ) < 0 \\
& g(1 - \alpha / \gamma) = - ( 2 \alpha (\gamma - \alpha) / \gamma ^2 ) ^ \beta < 0 \\
& g(1) = 0, ~ g'(1) = 0
\end{align*}

From $g'(\lambda)$, we know there exists a root $g(\lambda^{*}) = 0$ such that $\forall{0 < \lambda < \lambda^{*}}$, $g(\lambda) < 0$ and $\forall{\lambda^{*} < \lambda < 1}$, $g(\lambda) > 0$. Therefore, we can binary search $g(\lambda) = 0$ for a numerical solution $\lambda^{*} = 0.0160$.
So in this case, (\ref{eq:lambda}) holds if and only if $\lambda > \lambda^{*}$, i.e.
$v / u < \frac{1 - {\lambda^{*}}^2}{1 + {\lambda^{*}}^2} = 0.9995$.

Combining (a) and (b), $\Delta_{mean}^{mark} > \Delta_{mean}^{map}$ if and only if $v / u < 0.9995$.

The proof for $\Delta_{median}$ is similar. $\lambda^{*} = 0.0390$ and $\Delta_{median}^{mark} > \Delta_{median}^{map}$ if and only if $v / u < 0.9970$.

$\Delta_{tail}$ is different. As shown in Figure \ref{fig:lambda}, $\forall{0 < \lambda < 1}$, $g(\lambda) < 0$. So (\ref{eq:lambda}) never holds and $\Delta_{tail}^{mark} < \Delta_{tail}^{map}$.
\end{proof}

Although theoretically there are examples $\Delta_{mean}^{mark} < \Delta_{mean}^{map}$ (e.g. $\lambda = \frac{\gamma - \alpha}{\gamma}$). In practice, $v / u > 0.99$ should never happen (ground truth error being more than 99\% of validation error). Thus, we conclude that marking error has a larger impact on the mean and median, while map error has a larger impact on the tail.

\begin{figure}[t]
\centerline
{\includegraphics[width=0.5\textwidth]{figures/lambda.png}}
\caption{Algebraic function $g(\lambda)$ and its derivative $g'(\lambda)$.}
\label{fig:lambda}
\end{figure}

\subsection{Map Error (Scale)}
\label{sec:scale_error}

Besides the translation error, another type of map error is the scale error, which can be modeled by a linear transform
$\widehat{X}^{gt} = S X^{gt} + V$
where $S = diag[s_x, s_y]$ is a scaling matrix without rotation, and $V$ is a translation vector. Then
\begin{equation*}
Err^{map} = \widehat{X}^{gt} - X^{gt} = (S - I) X^{gt} + V
\end{equation*}
where $I$ is an identity matrix. For $S = I$, this reduces to the model we discussed in Section \ref{sec:map_error}.

Note that in this paper, our analysis only relies on the error distribution $Err^{gt}$. %
It does not require the distribution of ground truth location $X^{gt}$ (i.e. where the data is collected). With the scale error ($S \ne I$), the distribution of $Err^{map}$ depends on the distribution of $X^{gt}$. Unless $X^{gt}$ also follows a normal distribution and $s_x = s_y$, we cannot apply the same analysis in this paper. This additional distribution of $X^{gt}$ makes the model more complicated. We leave this as a topic for future work.

